Fast Doubly-Adaptive MCMC to Estimate the Gibbs Partition Function with Weak Mixing Time Bounds

We present a novel method for reducing the computational complexity of rigorously estimating the partition functions (normalizing constants) of Gibbs (Boltzmann) distributions, which arise ubiquitously in probabilistic graphical models. A major obstacle to practical applications of Gibbs distributions is the need to estimate their partition functions. The state of the art in addressing this problem is multi-stage algorithms, which consist of a cooling schedule, and a mean estimator in each step of the schedule. While the cooling schedule in these algorithms is adaptive, the mean estimation computations use MCMC as a black-box to draw approximate samples. We develop a doubly adaptive approach, combining the adaptive cooling schedule with an adaptive MCMC mean estimator, whose number of Markov chain steps adapts dynamically to the underlying chain. Through rigorous theoretical analysis, we prove that our method outperforms the state of the art algorithms in several factors: (1) The computational complexity of our method is smaller; (2) Our method is less sensitive to loose bounds on mixing times, an inherent component in these algorithms; and (3) The improvement obtained by our method is particularly significant in the most challenging regime of high-precision estimation. We demonstrate the advantage of our method in experiments run on classic factor graphs, such as voting models and Ising models.

==> badrange.tex <==

\begin{restatable}[Ranges of \superalgo~]{lemma}{lemma:schain-range}

\cyrus{Inconsistent $\Delta$ notation.}

\newcommand{\Range}{\operatorname{Range}}
\newcommand{\Hamiltonian}{\operatorname{H}}
\newcommand{\HMax}{\Hamiltonian_{\max}}
\newcommand{\HMin}{\Hamiltonian_{\min}}
Let $\Delta_{i} \doteq \frac{\beta_{i+1} - \beta_{i}}{2}$ and $\bar{\beta}_{i} \doteq \frac{\beta_{i+1} + \beta_{i}}{2}$.
Let $\Delta = \frac{\beta_{\max} - \beta_{\min}}{2}$

\[
\Range(f_{i}) = \Range(W_{i}) = \exp \left( -\Delta_{i} \HMin\right) - \exp \left( -\Delta_{i} \HMax\right) \leq 1 
\]

\[
\Range(g_{i}) = \Range(V_{i}) = \exp \left( \Delta_{i} \HMax\right) - \exp \left( \Delta_{i} \HMin\right) \leq ?
\]

Now, range of product $\neq$ product of range:

\[
\Range(V) = \left[ \prod_{i=1}^{\ell} \exp \left( \Delta_{i} \HMin\right), \ \prod_{i=1}^{\ell} \exp \left( \Delta_{i} \HMax\right) \right]
  = \left[ \exp \left(  \sum_{i=1}^{\ell} \Delta_{i} \HMin\right), \ \exp \left( \sum_{i=1}^{\ell} \Delta_{i} \HMax\right) \right] 
  = \left[ \exp \left( \Delta \HMin \right), \ \exp \left( \Delta \HMax\right) \right] 
  %\approx \left[ \prod_{i=1}^{\ell} \left(1 + \Delta_{i} \HMin\right), \ \prod_{i=1}^{\ell}  \left(1 +  \Delta_{i} \HMax \right) \right]
\]

Assuming $\HMin = 0$, this gives us
\[
\Range(V) = \left[1, \prod_{i=1}^{\ell} \exp \left( \Delta_{i} \HMax\right) \right]
\]

Now, note that $\exp(\delta \HMax) = $

Note also: $\lim_{\beta \to \infty} Z(\beta) = \exp(?)$.

Thus:

Note that $\mu = \frac{Z(0)}{Z(\beta)}$

So we get sample complexity range term:

\[
\approx \frac{\exp(\Delta \HMax)}{Q} = \frac{Z(\beta) \exp(\Delta \HMax)}{Z(0)}
\]

This begs the question: how does the contrapuntal movement of $Z(\beta)$ and $\exp(\Delta \HMax)$ behave?

Well:
\[
Q = \frac{Z(\beta)}{Z(0)} = ? \leq \exp(-\Hmin\beta)
\]

So worst case is when basically everything has Hamiltonian 0.

But at least one thing has $\HMax$!  So:
\[
Q \leq 
\]


If we assume instead $\HMin = 1$, we then get $Z(\beta) \leq Z_{0}\exp(-\beta)$.

In general
\[
Z(\beta) \leq Z(0)\exp(-\beta\HMin) \enspace.
\]

This gives range SC term
\[
\exp\left( -\beta\HMin \right) \left( \exp\left( \Delta\HMax \right) - \exp\left( \Delta\HMin \right) \right) = \exp\left( \Delta (\HMax - 2\HMin) \right) - \exp\left( -\Delta\HMin \right) =
\]

So, if $\Hamiltonian(x)$ is often $0$, it looks bad, because dividing $Q$ does nothing, but in general, it's a huge improvement.
Our algorithm doesn't work well for ``degenerate'' Gibbs samplers where this happens?

\[
 \mathcal{\tilde{O}}\left( \log(\delta^{-1})\left( \frac{\exp(\Delta)}{(1 - \EigTwoBound)Q\varepsilon} +(\varepsilon^{-2}) \cdot {\cal T}\cdot  \left(\RelITRelVar{\cal M}{\cal T}(f)+\RelITRelVar{\cal M}{\cal T}(g)\right)\right)\right)
\]

Kolmogorov algorithm gets $q \ln \beta / \varepsilon^{2}$.  So it all comes down to whether $Q$ is large (nondegenerate case).

How does $\frac{1}{1 - \Lambda}$ relate to $q \ln(n)$?



\end{restatable}


==> exp2.tex <==
For training Restricted Boltzmann Machines, it is important that we have a good estimate of the partition function $Z(\beta)=\sum{\exp(-\beta H(x))}$. Gibbs Sampling is used for estimating the partition function. The basic idea is that we are iterating through the hidden units $m^h$ and visible units $m^v$ in turn taking the other one determined. \\
The Hamiltonian function of an RBM equals $$\bold{E(v, h|\theta)= -v^TWh-b^Tv-a^Th}$$ 
And both the hidden and the visible units have binary values. In a single step of the Gibbs Sampler, we compute the probability of each hidden unit equal to 1 given all the visible unites observed, $$P(h_j = 1) = logistic(\beta b_j +\beta \sum_i w_{ij}v_i)$$
Then we update all the hidden units and compute the probability of each visible unit with $$P(v_i = 1) = logistic(\beta a_i +\beta \sum_j w_{ij}h_j)$$
That's basically how we are sampling from the RBM. 
There are other Gibbs Samplers introduced for estimating partition functions, with the most popular ones TAP(2015), AIS and RTS. The latter two include a cooling schedule. As the mixing rate are not analysed analytically for those methods (they simply stop when observing convergence) , we will stick with the original Gibbs Sampler so that our method that acquire the spectral gap can be applied. 
\sophia{I assume that we will have to use the spectral gap/ mixing time later?}


\paragraph{Problem with Constant Offsets}

\[
Z(\beta, H + c) = Z(\beta, H)\exp(-\beta c)
\]

Therefore, taking $c = -H_{\min}$ to ensure nonnegativity:
\[
\frac{Z(\beta_{\min}, H)}{Z(\beta_{\max}, H)} 
 = \frac{Z(\beta_{\min}, H - H_{\min})/\exp(\beta_{\min} H_{\min})}{Z(\beta_{\max}, H - H_{\min})/\exp(\beta_{\max} H_{\min})}
 = \frac{Z(\beta_{\min}, H - H_{\min})}{Z(\beta_{\max}, H - H_{\min})}\exp(\Delta H_{\min})
\]

So we can estimate $Q$ on the transformed chain, and it's a constant factor too big, but multiplicative error guarantees are the same.  This means TPA is slower?

==> paralelsudo.tex <==
\begin{algorithm}[H]\label{algo:paralgocode}
\algrenewcommand\algorithmicindent{1.0em}

\begin{algorithmic}
%\Procedure{\paralgo}{\dots} \small

%\State \textbf{input} $\{T_i\}_{i=1,2,\dots l}$, $H$, $\Omega$

\State $(\beta_0, \beta_1 ,\dots ,\beta_l)= \tpa(k,d)$
%\State $\Delta_i\gets \beta_{i+1}-\beta_i$
\State $ \varepsilon' \gets \frac{\sqrt[l]{1 + \varepsilon} - 1}{\sqrt[l]{1 + \varepsilon} + 1}$
\& $\delta'\gets \delta/2l$
\For{$i \in 1,2,\dots l $}
\State $f_i(x)= \exp(-\frac{\beta_{i+1}-\beta_i}{2}H(x))$
\State $g_{i-1}(x)= \exp(\frac{\beta_{i}-\beta_{i-1}}{2}H(x))$
\State $R_f=\exp(-\frac{\beta_{i+1}-\beta_i}{2}H_{\min})-\exp(-\frac{\beta_{i+1}-\beta_i}{2}H_{\max})$
\State $R_g=\exp(\frac{\beta_{i+1}-\beta_i}{2}H_{\max})-\exp(\frac{\beta_{i+1}-\beta_i}{2}H_{\min})$
\State  $\mu_i= \proc({\cal G}_i,   R_f, T_i, f_i, \varepsilon', \delta')$
\State $\nu_{i}= \proc({\cal G}_i,  R_g,T_i, g_{i}, \varepsilon', \delta')$
%\sophia{Are we starting a new chain here?}\cyrus{Yes}
\EndFor
 \State \textbf{return} $Z= \displaystyle \smash{\prod_{i=1}^l{\nu_i}/{\mu_i}}$

%\EndProcedure
\end{algorithmic}

%\vfill\columnbreak
%\end{multicols}
%\vspace{-0.5cm}
%\end{subfigure}
\caption{{\paralgo} }\label{algo:paralgocode}

\end{algorithm}
